Tight Space-Approximation Tradeoff for the Multi-Pass Streaming Set Cover Problem

We study the classic set cover problem in the streaming model: the sets that comprise the instance are revealed one by one in a stream and the goal is to solve the problem by making one or few passes over the stream while maintaining a sublinear space $o(mn)$ in the input size; here $m$ denotes the number of the sets and $n$ is the universe size. Notice that in this model, we are mainly concerned with the space requirement of the algorithms and hence do not restrict their computation time. Our main result is a resolution of the space-approximation tradeoff for the streaming set cover problem: we show that any $\alpha$-approximation algorithm for the set cover problem requires $\widetilde{\Omega}(mn^{1/\alpha})$ space, even if it is allowed polylog${(n)}$ passes over the stream, and even if the sets are arriving in a random order in the stream. This space-approximation tradeoff matches the best known bounds achieved by the recent algorithm of Har-Peled et.al. (PODS 2016) that requires only $O(\alpha)$ passes over the stream in an adversarial order, hence settling the space complexity of approximating the set cover problem in data streams in a quite robust manner. Additionally, our approach yields tight lower bounds for the space complexity of $(1- \epsilon)$-approximating the streaming maximum coverage problem studied in several recent works.

==> k-cover.tex <==
\subsection{The Lower Bound for the Distribution $\distSC$}\label{sec:hard-lower}

Throughout this section, fix $\protSC$ as a $\delta$-error protocol for \SetCover on the distribution $\distSC$. We first show that protocol 
$\protSC$ is essentially solving $m$ copies of the $\Disj_t$ problem on the distribution $\distDisj$ (for the parameter $t$ in the distribution $\distSC$) and then use a direct-sum style argument (similar in  
spirit to the ones in~\cite{BarakBCR10,Braverman12,BravermanR11}) to argue that the information cost of $\protSC$ shall  be $m$ times larger than the information
complexity of solving $\Disj_t$. However, to make the direct-sum argument work, we can only consider $\protSC$ on the distribution $\distSC \mid \theta = 0$, i.e., when \emph{all} underlying $\Disj_t$ instances
are sampled from $\distDisjN$. Consequently, we can only lower bound the information cost of $\protSC$ based on the information complexity of $\Disj_t$ on the distribution $\distDisjN$. 


\begin{lemma}\label{lem:direct-sum}
	There exists a $\paren{\delta+o(1)}$-protocol $\protDisj$ for $\Disjt$ on the distribution $\distDisj$ such that:
	\begin{enumerate}
	\item \label{part:ds-ic} $\ICost{\protDisj}{\distDisjN} = \frac{\Omega(1)}{m} \cdot \ICost{\protSC}{\distSC}$.
	\item \label{part:ds-cc} $\norm{\protDisj} = \norm{\protSC}$. 
	\end{enumerate}
\end{lemma}
\begin{proof}
	We design the protocol $\protDisj$ as follows: 
	\textbox{Protocol $\protDisj$. \textnormal{The protocol for solving $\Disjt$ using a protocol $\protSC$ for $\SetCover$.}}{
	\medskip
	\\ 
	\textbf{Input:} An instance $(A,B) \sim \distDisj$.  \textbf{Output:} \Yes if $A \cap B = \emptyset$ and \No otherwise. \\
	\algline
	
	\begin{enumerate}
		\item Using public randomness, the players sample an index $\istar \in_R [m]$ and $m$ mapping-extensions $f_1,\ldots,f_m$ independently and uniformly at random from $\FC$. 
		\item Using public randomness, the players sample the sets $A^{<\istar}$ and $B^{>\istar}$ each from $\distDisjN$ independently. 
		\item Using private randomness, Alice samples the sets $A^{>\istar}$ such that $(A_j,B_j) \sim \distDisjN$ (for all $j > \istar$); similarly Bob samples the sets $B^{<\istar}$. 
		\item The players construct the collections $\SS:= \set{S_1,\ldots,S_m}$ and $\ST:= \set{T_1,\ldots,T_m}$ by setting $S_i := [n] \setminus f_i(A_i)$ and $T_i:= [n] \setminus f_i(B_i)$ (exactly as in
		distribution $\distSC$).
		\item The players solve the \SetCover instance using \protSC and output \No iff $\protSC$ estimates $\opt(\SS,\ST) \leq 2\alpha$ and \Yes otherwise. 
	\end{enumerate}
	}

	It is easy to see that the distribution of instances $(\SS,\ST)$ created in the protocol $\protDisj$ matches the distribution $\distSC$ for \SetCover exactly. Moreover, by Lemma~\ref{lem:dist-sc-opt}, 
	$\opt(\SS,\ST) > 2\alpha$ w.p. $1-o(1)$, whenever $(A,B) \sim \distDisjN$ and $\opt(\SS,\ST) = 2$ whenever $(A,B) \sim \distDisjY$. Consequently, since $\protSC$ is an $\alpha$-approximation protocol,
	we have, 
	\begin{align*}
		\PR_{\distDisj}\paren{\protDisj~\errs} \leq \PR_{\distSC}\paren{\protSC~\errs} + o(1) \leq \delta + o(1)
	\end{align*}
	hence $\protDisj$ is indeed a $\paren{\delta+o(1)}$-error protocol for $\Disj$ on the distribution $\distDisj$. Moreover, it is clear that the communication cost of $\protDisj$ is at
	most the communication cost of \protSC. We now prove the bound on the information cost of this protocol. 
	
	Recall that our goal is to bound the information cost of $\protDisj$ whenever the instance $(A,B)$ is sampled from $\distDisjN$. Let $F$ be a random variable denoting the tuple $(f_1,\ldots,f_m)$,
	$I$ be a random variable for $\istar$ and $R$ be the set of public randomness used by the players. We know that, 
	\begin{align*}
		\ICost{\protDisj}{\distDisjN} = \II_{\distDisjN}(\protDisj : A \mid B,R) + \II_{\distDisjN}(\protDisj: B \mid A,R)
	\end{align*}
	We now bound the first term in the RHS above (the second term can be bounded exactly the same). 
	\begin{align*}
		\II_{\distDisjN}(\protDisj : A \mid B,R)&= {\II_{\distDisjN}(\protDisj : A \mid B,R,I)} \tag{$I$ is chosen using public randomness} \\
		&= \sum_{i=1}^{m} \Pr{I=i} \cdot \II_{\distDisjN}\paren{\protDisj : A_i \mid B_i,A^{<i},B^{>i},F,I=i} \tag{$R = (A^{<i},B^{>i},F)$} \\ 
		&= \sum_{i=1}^{m} \frac{1}{m} \cdot \II_{\distDisjN}\paren{\protDisj : A_i \mid B_i,A^{<i},B^{>i},F} 		%\\	&= \frac{1}{m} \sum_{i=1}^{m} \EX_{R \mid I=i} \bracket{I_{\distDisjN}(\protDisj;A \mid B,F,A^{<i},B^{>i})}
	\end{align*}
	where the last equality is true since conditioned on $(A,B) \sim \distDisjN$, all the chosen sets $A_j,B_j$ (for $j \in [m]$) are chosen from $\distDisjN$ and hence are independent of the $``I=i"$ event\footnote{We point out that
	this is the exact reason we need to consider information cost of $\protDisj$ on $\distDisjN$ (instead of $\distDisj$) as otherwise $(A_j,B_j)$'s are \emph{not} independent of $I = i$ and hence this equality would not hold.}. 
	Define $\bA:= (A_1,\ldots,A_m)$ and $\bB:= (B_1,\ldots,B_m)$; we can further derive, 
	\begin{align*}
		\II_{\distDisjN}(\protDisj : A \mid B,R) &= \sum_{i=1}^{m} \frac{1}{m} \cdot \II_{\distDisjN}\paren{\protDisj : A_i \mid B_i,A^{<i},B^{>i},F} \\
		&\leq \frac{1}{m} \cdot \sum_{i=1}^{m} \II_{\distDisjN}\paren{\protDisj : A_i \mid A^{<i},\bB,F} \tag{$A_i \perp B^{<i}$ and hence we can apply Fact~\ref{fact:info-increase}} \\
		&= \frac{1}{m} \cdot \II_{\distDisjN}\paren{\protDisj :  \bA \mid \bB,F} \tag{chain rule of mutual information: \itfacts{chain-rule}} \\
		&= \frac{1}{m} \cdot \II_{\distDisjN}\paren{\protDisj :  \SS \mid \ST,F} \tag{$\bA$ (resp. $\bB$) and $\SS$ (resp. $\ST$) uniquely determine each other conditioned on $F$} \\
		&= \frac{1}{m} \cdot \II_{\distSC}\paren{\protSC :  \SS \mid \ST,F,\theta=0} 
	\end{align*}
	where the last equality is because the distribution of set cover instances and the messages communicated by the players under $\distDisjN$ and under $\distSC \mid \theta = 0$ exactly matches. 
	
	Moreover, 
	\begin{align*}
		\II_{\distDisjN}(\protDisj : A \mid B,R) &\leq \frac{1}{m} \cdot \II_{\distSC}\paren{\protSC :  \SS \mid \ST,F,\theta=0} \\
		&\leq \frac{2}{m} \cdot \II_{\distSC}\paren{\protSC :  \SS \mid \ST,F,\theta} \tag{by definition of conditional mutual information as $\Pr{\theta = 0} = 1/2$} \\
		&\leq \frac{2}{m} \cdot \paren{\II_{\distSC}\paren{\protSC :  \SS \mid \ST,F} + H(\theta)} \tag{by Fact~\ref{fact:bar-hopping}}\\
		&= \frac{2}{m} \cdot \II_{\distSC}\paren{\protSC : \SS \mid \ST,F} + \frac{2}{m} \tag{$H(\theta) = 1$ by \itfacts{uniform}}  \\
		&\leq \frac{2}{m} \cdot \II_{\distSC}\paren{\protSC :  \SS \mid \ST} + \frac{2}{m} \tag{by data processing inequality (\itfacts{data-processing}), since $\protSC \perp F \mid \SS,\ST$}
	\end{align*}
	By performing the same exact calculation for $\II_{\distDisjN}(\protDisj : B \mid A,R)$, we obtain that, 
	\begin{align*}
		\ICost{\protDisj}{\distDisjN} &\leq \frac{2}{m} \cdot \paren{ \II_{\distSC}\paren{\protSC : \SS \mid \ST}  +  \II_{\distSC}\paren{\protSC : \ST \mid \SS} } + \frac{4}{m} \\
		&= \frac{2}{m} \cdot \ICost{\protSC}{\distSC} + \frac{4}{m} \\
		&= \frac{\Omega(1)}{m} \cdot \ICost{\protSC}{\distSC} 
%		&\leq \frac{2}{m} \cdot \HH_{\distSC}(\protSC \mid \theta=0) \leq \frac{2}{m} \cdot \norm{\protSC}
	\end{align*}
	where in the last inequality we used the fact that information cost of $\protSC$ is at least $1$. This finalizes the proof of the lemma. 
\end{proof}

Recall that in Lemma~\ref{lem:direct-sum}, we bound the information cost of $\protDisj$ on the distribution $\distDisjN$ (as opposed to $\distDisj$); in the following we prove that 
this weaker bound is still sufficient for our purpose. 

\begin{lemma}\label{lem:disjointness}
	For any $\delta < 1/2$, any $\delta$-error protocol $\protDisj$ for $\Disjt$ on $\distDisj$ with $\norm{\protDisj} = 2^{o(t)}$ has $\ICost{\protDisj}{\distDisjN} = \Omega(t)$. 
\end{lemma}

	By Theorem~\ref{thm:disjointness}, any $\delta$-error protocol for $\Disjt$ (with $\delta < 1/2$) on $\distDisj$ has $\ICost{\protDisj}{\distDisjY} = \Omega(t)$ (notice again that the information
	 cost is measured on the distribution $\distDisjY$). 
	From this, it is also relatively easy to obtain that 
	$\ICost{\protDisj}{\distDisj} = \Omega(t)$. However, to prove Lemma~\ref{lem:disjointness}, we need to lower bound the information cost
	of $\protDisj$ under the distribution $\distDisjN$. 
	
	To achieve this, we can relate  $\ICost{\protDisj}{\distDisjY}$ and $\ICost{\protDisj}{\distDisjN}$ to each other. The goal is to argue that if there is a large discrepancy in the information cost of $\protDisj$ 
	on $\distDisjY$ and $\distDisjN$, then the information cost of the protocol itself can be used to distinguish between these two cases. We can achieve this goal using a nice 
	construction of an ``information odometer'' by~\cite{BravermanW15}; informally speaking, the odometer allows the players to ``keep track'' of the amount of information revealed
	 in a protocol (i.e., the information cost of the protocol), while incurring a relatively small additional information cost overhead. 
	 
	Intuitively, we can use the odometer to argue that $\ICost{\protDisj}{\distDisjN} = \Theta(\ICost{\protDisj}{\distDisjY})$ as follows: suppose towards a contradiction that 
	$\ICost{\protDisj}{\distDisjN} = \tau$ for some $\tau = o(\ICost{\protDisj}{\distDisjY})$ and consider a new protocol $\protDisj'$ for $\Disj$ on $\distDisj$ which runs $\protDisj$ and the
	 information odometer for $\protDisj$ in parallel. Whenever
	the odometer estimates the information cost of $\protDisj$ to be larger than $c \cdot \tau$ (for some sufficiently large constant $c$), the players terminate the protocol and declare that the answer for $\Disj$ is $\No$
	(as information cost of $\protDisj$ on $\distDisjN$ is typically not much more than $\tau$, while its information cost on $\distDisjY$ is $\omega(\tau)$). If the cost
	is not estimated more than $c \cdot \tau$ by the end of the protocol, the players output the same answer as in $\protDisj$. As the information cost of the information odometer itself is bounded by $O(\tau)$, 
	this results in protocol $\protDisj'$ to have $\ICost{\protDisj'}{\distDisj} = o(t)$, a contradiction. This argument has been first made explicit in~\cite{GoosJP015}. 
	
	\begin{lemma}[Lemma 15 in \cite{GoosJP015}]\label{lem:one-sided-two-sided}
		Fix any function $F$, constants $0 < \eps_1 < \eps_2 < 1/2$, input distribution $\dist$, and define $\distN := \dist \mid F^{-1}(\No)$. 
		For every $\eps_1$-error protocol $\prot$ for $F$ on $\dist$, there exists an $\eps_2$-error protocol $\prot'$ for $F$ on $\dist$ such that: 
		\begin{align*}
			\ICost{\prot'}{\dist} = O\paren{\ICost{\prot}{\distN} + \log{\norm{\prot}}}
		\end{align*}
	\end{lemma}

	We are now ready to prove Lemma~\ref{lem:disjointness}. 

\begin{proof}[Proof of Lemma~\ref{lem:disjointness}]
	Let $\protDisj'$ be any $\delta'$-error protocol for $\Disj$ on $\distDisj$ for $\delta' < 1/2$. 
	We first prove that $\ICost{\protDisj'}{\distDisj} = \Omega(t)$ using the fact that $\ICost{\protDisj'}{\distDisjY} = \Omega(t)$ as follows: 
	\begin{align*}
		\ICost{\protDisj}{\distDisj} &= \II_{\distDisj}(\protDisj' : A \mid B) +  \II_{\distDisj}(\protDisj' : B \mid A) \\
		&\geq \II_{\distDisj}(\protDisj' : A \mid B,\theta) +  \II_{\distDisj}(\protDisj' : B \mid A,\theta) - 2\HH(\theta) \tag{by Fact~\ref{fact:bar-hopping}}\\
		&\geq \frac{1}{2} \cdot \paren{\II_{\distDisj}(\protDisj' : A \mid B,\theta = 0) +  \II_{\distDisj}(\protDisj' : B \mid A,\theta=0)} - 2 \tag{by definition of conditional mutual information and since $\HH(\theta) = 1$} \\
		&= \frac{1}{2} \cdot \paren{\II_{\distDisjY}(\protDisj' : A \mid B) +  \II_{\distDisjY}(\protDisj' : B \mid A)} - 2 \tag{$\distDisjY = \distDisj \mid \theta = 0$} \\
		&= \frac{1}{2} \cdot \ICost{\protDisj'}{\distDisjY} - 2 = \Omega(t) \tag{by Theorem~\ref{thm:disjointness}}
	\end{align*}
	
	Now suppose towards a contradiction that $\ICost{\protDisj}{\distDisjN} = o(t)$. We can then apply Lemma~\ref{lem:one-sided-two-sided} for the function $F = \Disj$, $\eps_1 = \delta$ and $\eps_2 = \delta' < 1/2$ to obtain 
	a protocol $\protDisj'$ with $\ICost{\protDisj'}{\distDisj} = O\paren{\ICost{\protDisj}{\distN} + \log{\norm{\protDisj}}} = o(t) + o(t) = o(t)$; a contradiction with the above bounds. 
\end{proof}

We now conclude: 

\begin{theorem}\label{thm:sc-cc-lower}
	For any constant $\delta < 1/2$, $\alpha = o(\frac{\log{n}}{\log{\log{n}}})$, and $m = \poly{(n)}$, 
	\begin{align*}
		\CC{\SetCover}{\distSC}{\delta} = \Omgt({mn^{\frac{1}{\alpha}}})
	\end{align*} 
\end{theorem}
\begin{proof}
	Let $t = \Theta\paren{(\frac{n}{\log{m}})^{\frac{1}{\alpha}}}$ and suppose towards a contradiction that there exists a $\delta$-error protocol $\protSC$ for $\SetCover$ on the 
	distribution $\distSC$ with $\norm{\protSC} = o(mt)$. By Lemma~\ref{lem:direct-sum}, this implies that there exists a $\paren{\delta+o(1)}$-error protocol $\protDisj$ for $\Disj$ on
	the distribution $\distDisj$ such that $\ICost{\protDisj}{\distDisjN} = o(t)$, and $\norm{\protDisj} = o(mt) \leq 2^{o(t)}$ (since $m = \poly(n)$ and $\alpha = o(\frac{\log{n}}{\log{\log{n}}})$). 
	However, this is in contradiction with Lemma~\ref{lem:disjointness}, implying that $\norm{\protSC} = \Omega(mt)$, hence proving the theorem. 
\end{proof}

As a corollary of Theorem~\ref{thm:sc-cc-lower}, we have that the space complexity of any $\alpha$-approximation streaming algorithm for set cover 
that uses $\polylog{(n)}$ many passes on \emph{adversarial streams} is $\Omgt({mn^{\frac{1}{\alpha}}})$. In the following section, we extend this result to random arrival streams. 


\newcommand{\distSCrnd}{\ensuremath{\distSC^{\textnormal{\textsf{rnd}}}}}

\newcommand{\Gstar}{\ensuremath{G^{\star}}}



\subsection{Extension to Random Arrival Streams}\label{sec:random-arrival}

In order to prove the lower bound in Theorem~\ref{thm:apx-lower} for random arrival streams, we need to relax the adversarial
 partitioning of the sets in the distribution $\distSC$, to a randomized partition.   



\textbox{Distribution \distSCrnd. {\textnormal{A random partitioning of the distribution $\distSC$}}} {

\begin{itemize}
	\item Sample the collections $(\SS,\ST) \sim \distSC$. 
	\item Assign each set in $\SS \cup \ST$ to Alice w.p. $1/2$ and the remainings to Bob.  
\end{itemize}
}

\begin{lemma}\label{lem:dist-random}
	For any constant $\delta < 1/4$, $\alpha = o(\log{n}/\log\log{n})$, and $m = \poly(n)$, 
	\begin{align*}
		\CC{\SetCover}{\distSCrnd}{\delta} = \Omgt(mn^{\frac{1}{\alpha}})
	\end{align*}
\end{lemma}
\begin{proof}
	Let $\SS = \set{S_1,\ldots,S_m}$ and $\ST = \set{T_1,\ldots,T_m}$ be the collections of sets sampled from $\distSC$ in the distribution $\distSCrnd$. For a sampled instance in $\distSCrnd$, we say that the index 
	$i \in [m]$ is \emph{good} iff $S_i$ is given to one player and $T_i$ to another. Let $G \subseteq [m]$ be the collection of all good indices. The index $\istar$ is chosen independent of the 
	random partitioning in $\distSCrnd$, and hence the probability that $\istar \in G$ is exactly $\card{G}/m$. Let $\event$ denote the event that $\card{G} \geq m/2 - o(m)$ and $i \in G$. We have, 
	\begin{align*}
		\Pr{\event} &= \Pr{\card{G} \geq m/2-o(m)} \cdot \Pr{\istar \in G \mid \card{G} \geq m/2-o(m)} \\
		&\geq \Pr{\card{G} \geq \paren{1-o(1)} \cdot \Ex{G}} \cdot \frac{1-o(1)}{2} \geq (1-o(1)) \cdot \frac{1}{2}
	\end{align*}
	
	Fix a $\delta$-error protocol $\protSC$ for \SetCover on the distribution $\distSCrnd$. Then, 
	\begin{align}
		\Pr{\protSC~\errs \mid \event} \leq \frac{\Pr{\protSC~\errs}}{\Pr{\event}} \leq 2\delta +o(1)\label{eq:prob-errs}
	\end{align}
	
	This in particular implies that there exists a set $\Gstar \subseteq [n]$ with $\card{\Gstar} \geq m/3$, such that conditioned on the set of good indices being 
	$\Gstar$ and conditioned on $\istar \in \Gstar$, the probability that $\protSC$ errs is at most $2\delta+o(1)$. Note that conditioned on the aforementioned events, the index $\istar$ is 
	chosen from $\Gstar$ uniformly at random. This implies that the distribution of the input given to Alice and Bob limited to the sets in $\Gstar$ matches the distribution $\distSC$ (with the number of the sets being 
	$2 \cdot \card{\Gstar}$ instead of $2m$). We can then use this to embed an instance of $\SetCover$ over the distribution $\distSC$ into the sets $\Gstar$ and obtain a protocol $\protSC'$ for $\distSC$. 
	
	More formally, the protocol $\protSC'$ works as follows: Given an instance $(\SS',\ST')$ sampled from $\distSC$ (with $\card{\SS'} = \card{\ST'} = \card{\Gstar}$), Alice and Bob use public coins to complete their input
	(i.e., increase the number of the sets to $2m$) by sampling from the distribution $\distSCrnd$ conditioned on $\Gstar$ (this is possible without any communication as the sets outside $\Gstar$ are sampled independent of the 
	 sets in $\Gstar$). The players then run the protocol $\protSC$ on this new instance and return the same answer as this protocol. As the distribution of the \SetCover instances sampled in the protocol $\protSC'$ matches
	 the distribution $\distSCrnd$ conditioned on $\Gstar$ and $\istar \in \Gstar$, by Eq~(\ref{eq:prob-errs}), the probability that $\protSC'$ errs is at most $2\delta+o(1)$. Since $\delta < 1/4$, we obtain a $\delta'$-error protocol 
	 for $\SetCover$ on the distribution $\distSC$ with $2\card{\Gstar}$ sets and universe of size $n$, for a constant $\delta' < 1/2$. Consequently, by Theorem~\ref{thm:sc-cc-lower}, 
	 $\norm{\protSC} = \norm{\protSC'} = \Omgt(\card{\Gstar} \cdot n^{\frac{1}{\alpha}}) = \Omgt(mn^{\frac{1}{\alpha}})$, proving the lemma.
\end{proof}

We are now ready to prove Theorem~\ref{thm:apx-lower}. 

\begin{proof}[Proof of Theorem~\ref{thm:apx-lower}]
	Fix a $p$-pass $s$-space streaming algorithm $\alg$ for the set cover problem over random arrival streams that outputs an $\alpha$-approximation w.p. at least $1-\delta$ for $\delta < 1/4$. One
	 can easily turn $\alg$ into a $\delta$-error protocol for $\SetCover$ on the distribution $\distSCrnd$: Alice and Bob take a random permutation of their inputs and then treat their combined input 
	 as a set stream and run $\alg$ on that. The random partitioning of the input plus the random permutation taken by the players ensure that the constructed stream is a random permutation of the input sets. Consequently,
	 this protocol is a $\delta$-error protocol for $\SetCover$ on $\distSCrnd$ that uses $p \cdot s$ bits of communication. Since $\delta < 1/4$, by Lemma~\ref{lem:dist-random}, $p \cdot s = \Omgt(mn^{\frac{1}{\alpha}})$, 
	 proving the theorem. 
\end{proof}


